Differentially Private AUC Computation in Vertical Federated Learning

Federated learning has gained great attention recently as a privacy-enhancing tool to jointly train a machine learning model by multiple parties. As a sub-category, vertical federated learning (vFL) focuses on the scenario where features and labels are split into different parties. The prior work on vFL has mostly studied how to protect label privacy during model training. However, model evaluation in vFL might also lead to potential leakage of private label information. One mitigation strategy is to apply label differential privacy (DP) but it gives bad estimations of the true (non-private) metrics. In this work, we propose two evaluation algorithms that can more accurately compute the widely used AUC (area under curve) metric when using label DP in vFL. Through extensive experiments, we show our algorithms can achieve more accurate AUCs compared to the baselines.

==> tables/evaluation_set_statistics_partial.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{|c|c|c|c|c|}\toprule
& $\#$ Positives ($P$) & $\#$ Negatives ($N$) & $\#$ Total ($M$) \\ \hline
 Criteo Evaluation Set &117,317 &341,090 &458,407 \\ 
\bottomrule
\end{tabular}}
\caption{Statistics of Criteo Evaluation Set}\label{tab:evaluation_set_statistics_criteo_partial}
\end{table*}

==> tables/top_k_analysis_production_data.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\setlength{\tabcolsep}{0.5em} % for the horizontal padding
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{c|c|c|c}\toprule
Top K & $\#$ Positives in Top K &Precision &Recall \\ \hline
1 &0 &0 &0 \\ \hline
5 &2 &0.4 &1.20e-3 \\ \hline
10 &2 &0.2 &1.20e-3 \\ \hline
50 &6 &0.12 &3.70e-3 \\ \hline
100 &13 &0.13 &8.00e-3 \\ \hline
500 &50 &0.1 &0.0306 \\ \hline
1,000 &94 &0.094 &0.0576 \\ \hline
5,000 &326 &0.0652 &0.1998 \\ \hline
10,000 &525 &0.0525 &0.3217 \\ \hline
50,000 &1,339 &0.0268 &0.8205 \\ \hline
100,000 &1,632 &0.0163 &1 \\
\bottomrule
\end{tabular}}
\caption{Top-k analysis on private data}\label{tab:top_k_analysis_production_data}
% \scriptsize
\end{table*}
